Combinatorial Analysis of Multiple Networks

The study of complex networks has been historically based on simple graph data models representing relationships between individuals. However, often reality cannot be accurately captured by a flat graph model. This has led to the development of multi-layer networks. These models have the potential of becoming the reference tools in network data analysis, but require the parallel development of specific analysis methods explicitly exploiting the information hidden in-between the layers and the availability of a critical mass of reference data to experiment with the tools and investigate the real-world organization of these complex systems. In this work we introduce a real-world layered network combining different kinds of online and offline relationships, and present an innovative methodology and related analysis tools suggesting the existence of hidden motifs traversing and correlating different representation layers. We also introduce a notion of betweenness centrality for multiple networks. While some preliminary experimental evidence is reported, our hypotheses are still largely unverified, and in our opinion this calls for the availability of new analysis methods but also new reference multi-layer social network data.

==> fig/dataset.tex <==

% \section{Terminology}
% \cite{Wasserman94} define the \emph{sociomatrix} of a relation $\mathcal{R}$ as a matrix with entries $x_{ij}$ representing the value of the tie from node  $i$ to node $j$ on relation $\mathcal{R}$. In their terminology, \emph{super-sociomatrix} is a collection of sociomatrices where each of them corresponds to one type of relation in a multi-layer network.
% 
% For our analyses, 

\subsection{Methodology}
%- population and sampling:
Collection of data was conducted at the Department of *** at *** University among the employees. The population of the study is 60 employees (out of the total number of 142) who decided to join the survey, including professors, postdoctoral researchers, PhD students and administration staff.

%- variables that we measured:
According to \cite{Wasserman94}, there are two types of variables that can be included in a network data set: \emph{structural} and \emph{composition} variables. Structural variables are measured on pairs of actors and they express specific ties between the pairs (e.g. friendship). Composition variables are defined for individual actors and they are measurements of various actor attributes (e.g. age). 

For our study, we measured 5 structural variables, namely: 
\begin{itemize}
\item current working relationships,  
\item repeated leisure activities,
\item regularly eating lunch together,
\item co-authorship of a publication,
\item and friendship on Facebook.
\end{itemize}
These variables cover different types of relations between the actors based on their \emph{interactions}. All relations are \emph{dichotomous} which means that they are either present or absent, without weights.
%TODO: if we have groups or ranks, we also have composition vars
%TODO: idea: how about adding information that we know about our group by hand??

%- collection process (offline):
Measurements of the first three variables (off-line data) were collected via a \emph{questionnaire} which had been distributed among the employees on-line. The questions were of a \emph{roster} format which means that each actor was presented with a complete list of other actors in the network and asked to select people with whom he/she has the aforementioned ties (working relationship, leisure activities, eating lunch). The number of choices for each question was not limited. The measurements are results of individual assessments done by the actors and therefore the relations are directed, however, we do not intend to study the aspect of personal perception of the relationships and so we decided to flatten the data into nondirectional connections. Thus, if an actor $A$ indicated a tie to actor $B$, we input an edge into the network even if actor $B$ did not indicate a tie to actor $A$.
On the top of this, the respondents were asked to provide their user information for a couple of most widespread online networks. 70\% of the respondents who filled in the questionnaire stated that they have a Facebook account and provided their username. All respondents provided answers to all questions which means that our multi-layer network is complete.
%In total, 50\% people responded to the survey and provided answers to all questions. This of course affects the accuracy of measurements, nevertheless, since we flatten all relations into nondirectional, the probability that we miss a tie is approximately 0.25. We do not claim that with such a collection we can perfectly reconstruct true relations in the population but the respondents who joined the survey provided information about all types of their ties which means that the multi-layer patterns in the network (if there are any) should be preserved.


%- collection process (online):
%TODO: is coauthorship online or offline?
Information about the co-authorship relation was obtained from the on-line DBLP bibliography database without the need to directly ask the actors. A co-authorship of at least one publication by a pair of actors resulted in an edge in the network. DBLP gets new data with a delay of several months and therefore the ``current working relationships" network is quite distinct from it. Moreover, ``current working relationships" network includes other types of interactions than cooperation on papers (e.g. also cooperation on administrative work).

Friendship relations among all the actors who stated that they have a Facebook account were retrieved from the site.
%TODO: what else can we say?

\subsection{Data Description}
We describe some common statistical measures of the single-layer networks in Tab.\,\ref{tabDataDescription}. The Co-authorship network is the smallest and less connected of all layers, Work and Lunch networks have the most edges and the highest average vertex degree can be observed for the Facebook network.

\begin{table}[t!] %\scriptsize
\begin{center}
\begin{tabular}{lccccc}
\hline
  &   \small{Work} &  \small{Leisure}  &  \small{Coauthor}  & \small{Lunch} &  \small{FB} \\
\hline
 \small{\# of edges}  &   194  &  88 &  21 &  193 &   124 \\
\small{\# of con. comp.} &  2   &  1   &   8 &   1  &   1    \\
 \small{avg. vertex deg.} &  $6.47$ &   $3.74$  &  $1.68$ &  $6.43$ &   $7.75$   \\ 
\hline
\end{tabular}
\caption{Basic statistics computed on the sociomatrices of the 5 different relations---number of edges, number of connected components and average vertex degree.} 
\label{tabDataDescription}
\end{center}
\end{table}

The analysis of the network through a super-sociomatrix approach has been for a long time a viable approach to handle multiple networks. 
%With this perspective each layer of the super-sociomatrix is the sociomatrix for one of the relations \cite{Wasserman1994}. 
In the multi-layer super-sociomatrix, all the layers componing our complex structure of experience are merged together producing a single layer network. We can therefore produce a summary description of this network. It counts 61 nodes and 706 edges belonging to all the 5 layers we are using in this study. Average vertex degree is $11.57$ and the network has a diameter of 4. Using a modularity algorithm, it is possible to detect 5 different clusters with a network modularity value of $0.41$. % and clustering coefficient of $0.069$.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{fig/supersociomatrix.pdf}
\caption{Visualization of the super-sociomatrix.}
\label{fig_toyCluster}
\end{figure}


%%%%%%%% TODO: belongs to coverage.tex




\begin{table}[t!] %\scriptsize
\begin{center}
\begin{tabular}{|l|c|r|}
%\hline
%  &   \small{Work} &  \small{Leisure}  &  \small{Coauthor}  & \small{Lunch} &  \small{FB} \\
\hline
 $\mathcal{R}$ & \small{Covering combination of layers} & \small{Prob.} \\
\hline
 Coauthor  & Work, Leisure, FB  & 0.95 \\
 Coauthor  & Work, Leisure & 0.90 \\
 Coauthor  & Work & 0.86 \\
 Leisure &  Work, Coauthor, Lunch, FB   & 0.89 \\
 Leisure &  Work, Lunch   & 0.78 \\
 Lunch &  Work, Leisure, Coauthor, FB & 0.70\\
 Work &  Leisure, Coauthor, Lunch, FB & 0.66\\  
 FB &  Work, Leisure, Coauthor, Lunch & 0.64\\  
\hline
\end{tabular}
\caption{Best covering combinations of layers for each single network. In fact, this was computed as conditional probability that there is an edge in the combination of layers in case that there is an edge in the single network.} 
\label{tabProb}
\end{center}
\end{table}


\begin{table}[t!] %\scriptsize
\begin{center}
\begin{tabular}{|l|c|r|}
%\hline
%  &   \small{Work} &  \small{Leisure}  &  \small{Coauthor}  & \small{Lunch} &  \small{FB} \\
\hline
 $\mathcal{R}$& \small{Similar combination of layers} & \small{Jaccard}\\
\hline
 Lunch &  Work, Leisure & 0.39\\
 Work &  Coauthor, Lunch & 0.36\\  
 Leisure &  Coauthor, Lunch   & 0.27 \\
 FB &  Work, Leisure, Lunch & 0.23\\
 Coauthor  & Leisure, FB  & 0.07 \\  
\hline
\end{tabular}
\caption{Each layer compared to the most similar combination of other layers.} 
\label{tabJaccard}
\end{center}
\end{table}


%TODO: figure from between.
\begin{figure*}
\centering
\includegraphics[width=0.9\textwidth]{fig/between_rank.pdf}
\caption{Increase/decrease of 61 individual actors in ranking according to two different measures of betweenness. Actors were sorted (from left to right) in a descending order according to the traditional measure of betweenness calculated on the super-sociomatrix. Then, betweenness was recalculated using the new multi-layer distance and increase/decrease in ranking of each actor (compared to the traditional measure) was plotted.}
\label{fig_defSociomatrix}
\end{figure*}

% facebook | work leisure lunch 	0.227273
% 
% lunch | work leisure coauthor 	0.38835
% -lunch | work leisure 	0.386364
% 
% coauthor lunch facebook | work 	0.364431
% -coauthor lunch | work 	0.362069
% 
% 
% -coauthor lunch | leisure 	0.278761
% lunch | leisure 	0.277273
% 
% -leisure facebook | coauthor 	0.0736842









==> supersociomatrix.tex <==


%\section{supersociomatrix}
The analysis of the network through a supers-ociomatrix approach has been for a long time a viable approach to handle multiple networks. With this perspective  each layer of the super-sociomatrix is the sociomatrix for one of the relations \cite{Wasserman1994}. In the super-sociomatrix all the layers componing our complex structure of experience are merged together producing a single layer network. We can therefore produce a summary description of this network. It counts 61 nodes and 706 edges belonging to the 5 layers we are using in this study. Average degree is 11,57 and the network has a diameter of 4.  Using a modularity algorithm is possible to detect 5 different clusters with a network modularity value of 0,41 and clustering coefficient for the whole network is 0,069





